Information Bottleneck and its Applications in Deep Learning

Information Theory (IT) has been used in Machine Learning (ML) from early days of this field. In the last decade, advances in Deep Neural Networks (DNNs) have led to surprising improvements in many applications of ML. The result has been a paradigm shift in the community toward revisiting previous ideas and applications in this new framework. Ideas from IT are no exception. One of the ideas which is being revisited by many researchers in this new era, is Information Bottleneck (IB); a formulation of information extraction based on IT. The IB is promising in both analyzing and improving DNNs. The goal of this survey is to review the IB concept and demonstrate its applications in deep learning. The information theoretic nature of IB, makes it also a good candidate in showing the more general concept of how IT can be used in ML. Two important concepts are highlighted in this narrative on the subject, i) the concise and universal view that IT provides on seemingly unrelated methods of ML, demonstrated by explaining how IB relates to minimal sufficient statistics, stochastic gradient descent, and variational auto-encoders, and ii) the common technical mistakes and problems caused by applying ideas from IT, which is discussed by a careful study of some recent methods suffering from them.

==> blind_unsafe.tex <==
\newcommand{\authorsData}{{\large Hassan Hafez-Kolahi\\}
{\small Department of Computer Engineering, Sharif University of Technology, Tehran, Iran\\}
hafez@ce.sharif.edu\\
{\large Shohreh Kasaei*\\}
{\small Department of Computer Engineering, Sharif University of Technology, Tehran, Iran\\
skasaei@sharif.edu}}

\newcommand \authorsBio {\vskip 1.5cm
%\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/hassan.jpg}}]{Hassan Hafez-Kolahi}
\textbf{Hassan Hafez-Kolahi}
was born in Mashhad, Iran, in 1989. He received the B.Sc. degree in Computer Engineering from Ferdowsi University of Mashhad in 2011, the M.Sc. degree in 2013 from Sharif University of Technology. He is currently a Ph.D. candidate at Sharif University of Technology. His research interests are in machine learning and information theory.
%%\end{IEEEbiography}
%\end{biography}

\vskip 0.5cm
%\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/skasaei.jpg}}]{Shohreh Kasaei}
\textbf{Shohreh Kasaei}
received the B.Sc. degree from the Department of Electronics, Faculty of Electrical and Computer Engineering, Isfahan University of Technology, Iran, in 1986, the M.Sc. degree from the Graduate School of Engineering, Department of Electrical and Electronic Engineering, University of the Ryukyus, Japan, in 1994, and the Ph.D. degree from Signal Processing Research Centre, School of Electrical and Electronic Systems Engineering, Queensland University of Technology, Australia, in 1998. She joined Sharif University of Technology since 1999, where she is currently a full professor and the director of Image Processing Laboratory (IPL). Her research interests are in 3D computer vision and image/video processing including dynamic 3D object tracking, dynamic 3D human activity recognition, virtual reality, 3D semantic segmentation, multi-resolution texture analysis, scalable video coding, image retrieval, video indexing, face recognition, hyperspectral change detection, video restoration, and fingerprint authentication.
%\end{IEEEbiography}
}

\newcommand \AcknowledgmentText{We wish to thank Dr. Mahdieh Soleymani for her beneficial discussions and comments.}
